PrimitiveAnything: Human-Crafted 3D Primitive Assembly Generation with Auto-Regressive Transformer

Shape primitive abstraction, which decomposes complex 3D shapes into simple geometric elements, plays a crucial role in human visual cognition and has broad applications in computer vision and graphics. While recent advances in 3D content generation have shown remarkable progress, existing primitive abstraction methods either rely on geometric optimization with limited semantic understanding or learn from small-scale, category-specific datasets, struggling to generalize across diverse shape categories. We present PrimitiveAnything, a novel framework that reformulates shape primitive abstraction as a primitive assembly generation task. PrimitiveAnything includes a shape-conditioned primitive transformer for auto-regressive generation and an ambiguity-free parameterization scheme to represent multiple types of primitives in a unified manner. The proposed framework directly learns the process of primitive assembly from large-scale human-crafted abstractions, enabling it to capture how humans decompose complex shapes into primitive elements. Through extensive experiments, we demonstrate that PrimitiveAnything can generate high-quality primitive assemblies that better align with human perception while maintaining geometric fidelity across diverse shape categories. It benefits various 3D applications and shows potential for enabling primitive-based user-generated content (UGC) in games. Project page: https://primitiveanything.github.io

==> sec/6_figureonly.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=0.98\linewidth]{images/comp_main2.png}
% \vspace{-20pt}
\caption{More qualitative comparisons with optimization-based methods on the HumanPrim dataset.
}
\label{fig:main2}
% \vspace{-10pt}
\end{figure*}


\begin{figure*}[htb]
\centering
\begin{minipage}[t]{0.48\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{images/comp_chair.png}
    \caption{Comparisons on the HumanPrim test set (Chair subset).}
    \label{fig:chair}
\end{minipage}%
%\hspace{4pt}
\quad
\begin{minipage}[t]{0.49\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{images/shapenet.png}
    \caption{Comparisons on the ShapeNet test set (Chair category).}
    \label{fig:shapenet}

\end{minipage}
\end{figure*}


\begin{figure*}[t]
\centering
\includegraphics[width=0.93\linewidth]{images/comp_objaverse.png}
\vspace{-2pt}
\caption{
Comparisons on the Objaverse dataset.
}
\label{fig:objaverse}
% \vspace{-10pt}
\end{figure*}


\begin{figure*}[t]
\centering
\includegraphics[width=0.93\linewidth]{images/app2.png}
% \vspace{-5pt}
\caption{
More visualizations of primitive-based 3D content generation on text and image conditions.
}
\label{fig:app2}
% \vspace{-10pt}
\end{figure*}
